Learning Quantum Processes with Quantum Statistical Queries

In this work, we initiate the study of learning quantum processes from quantum statistical queries. We focus on two fundamental learning tasks in this new access model: shadow tomography of quantum processes and process tomography with respect to diamond distance. For the former, we present an efficient average-case algorithm along with a nearly matching lower bound with respect to the number of observables to be predicted. For the latter, we present average-case query complexity lower bounds for learning classes of unitaries. We obtain an exponential lower bound for learning unitary 2-designs and a doubly exponential lower bound for Haar-random unitaries. Finally, we demonstrate the practical relevance of our access model by applying our learning algorithm to attack an authentication protocol using Classical-Readout Quantum Physically Unclonable Functions, partially addressing an important open question in quantum hardware security.

==> content/sim.tex <==
\label{sec:simulations}

In this section, we demonstrate the performance of our learning algorithm presented in this work through simulations. Our simulation results allow us to apply our algorithms to learn processes. The code for our simulations is available in a public Github repository \footnote{\url{https://github.com/chirag-w/qpsq-learning}}. Before presenting our simulation result, we give a remark on our approach for providing a good and realistic simulation of data obtained via statistical queries. In order to construct the output of the statistical query oracles in our simulations, we assume the oracle \textit{QPStat} uses a method to estimate the expectation value of an observable, such as the ones shown in \cite{classical_shadow_tomography, hadfield2020measurements_locally_biased, Huang_2021_derandom, Wu2023overlappedgrouping}. In our simulation, in order to emulate the behaviour of these methods, we compute the true expectation value and output the result after adding a normally distributed error to it. The error is sampled from a normal distribution such that it is within the specified tolerance with high probability. We note that our learning model puts no assumptions on the error in the output of the queries, and in theory, this error can come from any arbitrary distribution as long as it is within the tolerance with high probability. However, we will argue that this simple method of generating the sample data already captures these scenarios well enough for the purpose of the simulation. We also compare this method with the use of classical shadows for evaluating the outcome of an observable \cite{classical_shadow_tomography} in Fig \ref{fig:compare-cs-norm}. We see that for the same target tolerance and success probabilities, the classical shadow method produces less error than that generated using a normal distribution. In fact, the normally distributed error achieves the exact value for the success probability, while any practical method would produce the same error or less, as it would come with a bound that may not be tight. Thus, our emulated oracle would produce greater deviations than in a practical implementation, implying that the real-life performance of the algorithm would only be similar to or better than the simulations. We use these emulated oracles for the simulation of the learning algorithms.
\begin{figure}
\centering
\includegraphics[width=0.42\textwidth]{images/compare-norm-cs.png}
\caption{\small Comparison between simulated errors generated from a normal distribution and those generated by using classical shadow tomography to evaluate the EV of the Pauli-Z observable on random single-qubit stabilizer states after evolution under a fixed haar-random unitary. We fix a tolerance value $\tau = 0.2$, and the probability of the deviation lying outside the tolerance, $\delta = 0.0455$}
\label{fig:compare-cs-norm}
\end{figure}

In figure \ref{fig:learn-arb-alg-haar}, we show the simulated performance of algorithm \ref{alg:sq-arb-proc} in learning 10 haar-random unitaries over 6 qubits for a range of tolerances. We consider $O = Z \otimes I ... \otimes I$, the Pauli-Z observable on the first qubit. We consider three distributions of target states, namely the uniform distributions over the computational basis states, the stabilizer product states and haar-random states. We can see from figure \ref{fig:learn-arb-alg-haar} that a lower QPSQ tolerance results in a lower prediction error for the same number of queries. We also see that the algorithm achieves similar performance when predicting the outcome on computational basis and stabilizer product states, even though the uniform distribution over the computational basis states is not locally flat and thus outside the performance guarantee. On the other hand, the distribution over haar-random states is within the guarantee, and the algorithm performs best on this distribution.
\begin{figure}[H]
    \vspace{-1em}
     \centering
     \begin{subfigure}[b]{0.42\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/sq-sim/haar-unitaries-comp-distr.png}
         \caption{Computational basis states}
         \label{fig:haar-error-classical}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.42\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/sq-sim/haar-unitaries-stab-distr.png}
         \caption{Stabilizer states}
         \label{fig:haar-error-stab}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.42\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/sq-sim/haar-unitaries-haar-distr.png}
         \caption{Haar-random states}
         \label{fig:haar-error-haar}
     \end{subfigure}
        \caption{Average performance of the learning algorithm on 10 haar-random 6-qubit unitaries, in predicting the outcome of $Z_1$ on three target distributions}
        \label{fig:learn-arb-alg-haar}
    \vspace{-1em}
\end{figure}

